Balancing Work and Size with Bounded Buffers

We consider the fundamental problem of managing a bounded size queue buffer where traffic consists of packets of varying size, where each packet requires several rounds of processing before it can be transmitted from the queue buffer. The goal in such an environment is to maximize the overall size of packets that are successfully transmitted. This model is motivated by the ever-growing ubiquity of network processors architectures, which must deal with heterogeneously-sized traffic, with heterogeneous processing requirements. Our work addresses the tension between two conflicting algorithmic approaches in such settings: the tendency to favor packets with fewer processing requirements, thus leading to fast contributions to the accumulated throughput, as opposed to preferring packets of larger size, which imply a large increase in throughput at each step. We present a model for studying such systems, and present competitive algorithms whose performance depend on the maximum size a packet may have, and maximum amount of processing a packet may require. We further provide lower bounds on algorithms performance in such settings.

==> graphs/B.k10.l005.L10.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 11.99)
(60.000000, 17.43)
(70.000000, 23.48)
(80.000000, 29.65)
(90.000000, 35.99)
(100.000000, 42.69)
(110.000000, 49.91)
(120.000000, 57.40)
(130.000000, 64.90)
(140.000000, 72.76)
(150.000000, 80.65)
(160.000000, 88.39)
(170.000000, 96.18)
(180.000000, 104.36)
(190.000000, 112.10)
(200.000000, 119.77)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 13.28)
(60.000000, 18.99)
(70.000000, 25.20)
(80.000000, 31.33)
(90.000000, 37.52)
(100.000000, 43.80)
(110.000000, 50.59)
(120.000000, 57.64)
(130.000000, 65.36)
(140.000000, 73.43)
(150.000000, 81.75)
(160.000000, 90.28)
(170.000000, 98.74)
(180.000000, 107.87)
(190.000000, 116.39)
(200.000000, 124.97)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 12.04)
(60.000000, 16.88)
(70.000000, 22.14)
(80.000000, 27.73)
(90.000000, 32.98)
(100.000000, 37.37)
(110.000000, 40.84)
(120.000000, 44.16)
(130.000000, 47.94)
(140.000000, 51.93)
(150.000000, 56.03)
(160.000000, 60.17)
(170.000000, 64.56)
(180.000000, 68.99)
(190.000000, 73.18)
(200.000000, 77.71)
};


==> graphs/B.k10.l005.L10.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 1)
(60, 1)
(70, 1)
(80, 1)
(90, 1)
(100, 1)
(110, 1)
(120, 1)
(130, 1)
(140, 1)
(150, 1)
(160, 1)
(170, 1)
(180, 1)
(190, 1)
(200, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.943513382155479)
(60, 0.973505718662158)
(70, 0.986179522434171)
(80, 0.992068183607024)
(90, 0.995150230939442)
(100, 0.996810569473171)
(110, 0.997830318103257)
(120, 0.998445433595538)
(130, 0.998871454389549)
(140, 0.999151181355353)
(150, 0.999336692939116)
(160, 0.999473306037016)
(170, 0.999572938104496)
(180, 0.999641632334621)
(190, 0.999689975438768)
(200, 0.999728710481876)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.885420740899393)
(60, 0.925832871401441)
(70, 0.946421952862349)
(80, 0.957491061948608)
(90, 0.96352208952278)
(100, 0.966814404874627)
(110, 0.969055396615342)
(120, 0.970610780444121)
(130, 0.971877854636748)
(140, 0.973059814614102)
(150, 0.973949087114707)
(160, 0.974666296988358)
(170, 0.975157687520845)
(180, 0.975481014647363)
(190, 0.975723580409571)
(200, 0.97593427767458)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.877497549282084)
(60, 0.899424197796503)
(70, 0.907749968350051)
(80, 0.911455729089271)
(90, 0.913475885322235)
(100, 0.914661747094639)
(110, 0.915543201644384)
(120, 0.91601286450112)
(130, 0.916017614558694)
(140, 0.916229005573556)
(150, 0.916310860579072)
(160, 0.916244270148932)
(170, 0.916284805544484)
(180, 0.916338800107624)
(190, 0.916358431334277)
(200, 0.916361018688888)
};


==> graphs/B.k10.l005.L10.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.924173228370435)
(60, 0.928425888452711)
(70, 0.930888563861616)
(80, 0.932420922295846)
(90, 0.933422345330616)
(100, 0.934116048135301)
(110, 0.934614856385553)
(120, 0.934979065584149)
(130, 0.935253136051321)
(140, 0.935468433629421)
(150, 0.935641098023739)
(160, 0.935780721700626)
(170, 0.935897353910544)
(180, 0.935999064506139)
(190, 0.936087680623857)
(200, 0.936165790707001)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.871969808397336)
(60, 0.903827911762709)
(70, 0.91802323934848)
(80, 0.925025130739226)
(90, 0.928895462519798)
(100, 0.931136749895777)
(110, 0.932587039451226)
(120, 0.933525578539917)
(130, 0.93419766022997)
(140, 0.934674390581477)
(150, 0.935020480676966)
(160, 0.935287851643829)
(170, 0.935497667812586)
(180, 0.935663632706595)
(190, 0.935797470451397)
(200, 0.935911818740756)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.818282144583134)
(60, 0.859567206189607)
(70, 0.881013372507139)
(80, 0.89278469907215)
(90, 0.899373048580208)
(100, 0.903116851161769)
(110, 0.905693570337292)
(120, 0.907500760545546)
(130, 0.908951811407848)
(140, 0.910266740604788)
(150, 0.911266793287222)
(160, 0.912073930813042)
(170, 0.912647499396284)
(180, 0.913049317153431)
(190, 0.913362823315601)
(200, 0.91363628473729)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.810959743007168)
(60, 0.835048709935085)
(70, 0.845014064382807)
(80, 0.84986039154925)
(90, 0.852658803280441)
(100, 0.854400216576574)
(110, 0.855680277919635)
(120, 0.856452852114317)
(130, 0.856708346694269)
(140, 0.857103312689737)
(150, 0.85733809972328)
(160, 0.857403724374031)
(170, 0.85754852493752)
(180, 0.857692259671414)
(190, 0.857791838607819)
(200, 0.857865837633956)
};


==> graphs/B.k10.l005.L15.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 5.13)
(60.000000, 7.53)
(70.000000, 10.55)
(80.000000, 14.04)
(90.000000, 17.95)
(100.000000, 22.09)
(110.000000, 26.41)
(120.000000, 30.80)
(130.000000, 35.16)
(140.000000, 39.76)
(150.000000, 44.65)
(160.000000, 49.57)
(170.000000, 54.69)
(180.000000, 59.91)
(190.000000, 65.26)
(200.000000, 70.92)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 5.77)
(60.000000, 8.46)
(70.000000, 11.60)
(80.000000, 15.13)
(90.000000, 19.05)
(100.000000, 23.16)
(110.000000, 27.43)
(120.000000, 31.68)
(130.000000, 35.91)
(140.000000, 40.33)
(150.000000, 44.77)
(160.000000, 49.49)
(170.000000, 54.37)
(180.000000, 59.57)
(190.000000, 64.80)
(200.000000, 70.30)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 5.58)
(60.000000, 7.91)
(70.000000, 10.69)
(80.000000, 13.84)
(90.000000, 17.22)
(100.000000, 20.79)
(110.000000, 24.57)
(120.000000, 28.40)
(130.000000, 32.01)
(140.000000, 35.22)
(150.000000, 37.87)
(160.000000, 40.42)
(170.000000, 42.73)
(180.000000, 45.16)
(190.000000, 47.73)
(200.000000, 50.21)
};


==> graphs/B.k10.l005.L15.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 1)
(60, 1)
(70, 1)
(80, 1)
(90, 1)
(100, 1)
(110, 1)
(120, 1)
(130, 1)
(140, 1)
(150, 1)
(160, 1)
(170, 1)
(180, 1)
(190, 1)
(200, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.70610371043685)
(60, 0.863340100802545)
(70, 0.925282046269769)
(80, 0.956617844263892)
(90, 0.973696427857851)
(100, 0.98327835265696)
(110, 0.988790009127104)
(120, 0.992220515531414)
(130, 0.994438032140406)
(140, 0.995893281128384)
(150, 0.99689518550664)
(160, 0.997609198223045)
(170, 0.998113824460108)
(180, 0.998504036637166)
(190, 0.9987895752545)
(200, 0.99901022110263)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.655845286795786)
(60, 0.801139304351465)
(70, 0.86439541901152)
(80, 0.902625456700622)
(90, 0.927215117409383)
(100, 0.942741592763099)
(110, 0.952869029240638)
(120, 0.959463267662936)
(130, 0.964031237632516)
(140, 0.967123809770477)
(150, 0.969353682157784)
(160, 0.970986109523106)
(170, 0.972308436202794)
(180, 0.973385163963404)
(190, 0.97433830429737)
(200, 0.975177178892756)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.677145764076472)
(60, 0.808376357700771)
(70, 0.859582341578668)
(80, 0.883395719869801)
(90, 0.895474803195213)
(100, 0.901747927258565)
(110, 0.905322264439416)
(120, 0.907397038421335)
(130, 0.908737058089517)
(140, 0.909755784974317)
(150, 0.910650884008442)
(160, 0.911216511290021)
(170, 0.9116309920699)
(180, 0.911802490916131)
(190, 0.91180028693944)
(200, 0.912063254907018)
};


==> graphs/B.k10.l005.L15.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.911578199065037)
(60, 0.921077374757269)
(70, 0.926841454962383)
(80, 0.930521778125379)
(90, 0.932996586521735)
(100, 0.934717149644064)
(110, 0.935959214202516)
(120, 0.93687243536185)
(130, 0.937560493047266)
(140, 0.938095544297615)
(150, 0.938519689446159)
(160, 0.938855759021881)
(170, 0.939125641008992)
(180, 0.939347557939798)
(190, 0.93953187780682)
(200, 0.939686874058633)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.643668748713165)
(60, 0.795203033569884)
(70, 0.857589758015244)
(80, 0.890153737430904)
(90, 0.908455443499782)
(100, 0.919087139102224)
(110, 0.925467119953903)
(120, 0.929584050801907)
(130, 0.932345811718513)
(140, 0.934243049622469)
(150, 0.935605759912063)
(160, 0.936611141004908)
(170, 0.937354285196036)
(180, 0.937942328408153)
(190, 0.938394645172736)
(200, 0.938756791820555)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.597854265402595)
(60, 0.737911287266911)
(70, 0.801157507819456)
(80, 0.839912644950295)
(90, 0.865088539514305)
(100, 0.881196734438429)
(110, 0.891846547845981)
(120, 0.898894688215614)
(130, 0.903837602467708)
(140, 0.907254536729818)
(150, 0.909757516742213)
(160, 0.911615900856019)
(170, 0.9131197834074)
(180, 0.914346976703854)
(190, 0.915421896655621)
(200, 0.916361194887051)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.617271316121349)
(60, 0.744577173366868)
(70, 0.796696548128745)
(80, 0.822018956041597)
(90, 0.835474934697356)
(100, 0.842879252264569)
(110, 0.847344715224758)
(120, 0.850115273225927)
(130, 0.85199596423273)
(140, 0.853437848283385)
(150, 0.854663784853473)
(160, 0.855500869340464)
(170, 0.856136039791308)
(180, 0.856499443165493)
(190, 0.856665435773009)
(200, 0.857053868947318)
};


==> graphs/B.k10.l005.L25.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 3.45)
(60.000000, 3.93)
(70.000000, 4.38)
(80.000000, 5.29)
(90.000000, 6.43)
(100.000000, 7.61)
(110.000000, 8.73)
(120.000000, 9.73)
(130.000000, 10.56)
(140.000000, 11.21)
(150.000000, 11.72)
(160.000000, 12.12)
(170.000000, 12.38)
(180.000000, 12.60)
(190.000000, 12.75)
(200.000000, 12.90)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 3.46)
(60.000000, 4.05)
(70.000000, 4.67)
(80.000000, 5.72)
(90.000000, 7.00)
(100.000000, 8.26)
(110.000000, 9.48)
(120.000000, 10.61)
(130.000000, 11.57)
(140.000000, 12.38)
(150.000000, 13.07)
(160.000000, 13.62)
(170.000000, 14.08)
(180.000000, 14.46)
(190.000000, 14.74)
(200.000000, 14.96)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50.000000, 3.95)
(60.000000, 4.22)
(70.000000, 4.54)
(80.000000, 5.29)
(90.000000, 6.21)
(100.000000, 7.09)
(110.000000, 7.88)
(120.000000, 8.57)
(130.000000, 9.13)
(140.000000, 9.57)
(150.000000, 9.92)
(160.000000, 10.20)
(170.000000, 10.42)
(180.000000, 10.56)
(190.000000, 10.70)
(200.000000, 10.82)
};


==> graphs/B.k10.l005.L25.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 1)
(60, 1)
(70, 1)
(80, 1)
(90, 1)
(100, 1)
(110, 1)
(120, 1)
(130, 1)
(140, 1)
(150, 1)
(160, 1)
(170, 1)
(180, 1)
(190, 1)
(200, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.00166933981385907)
(60, 0.14064061638302)
(70, 0.51439558622449)
(80, 0.766186631452798)
(90, 0.867735328729381)
(100, 0.938785348750787)
(110, 0.966203861234895)
(120, 0.983440266419412)
(130, 0.991237425771225)
(140, 0.99546602099722)
(150, 0.99758025192907)
(160, 0.99868853524237)
(170, 0.999229097865431)
(180, 0.999555013744179)
(190, 0.999725387204681)
(200, 0.999824770202749)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.00161747505363822)
(60, 0.124922663260813)
(70, 0.491618476075805)
(80, 0.757387781444179)
(90, 0.846845513977546)
(100, 0.918539667804214)
(110, 0.948495625343994)
(120, 0.97030826846702)
(130, 0.981580249206813)
(140, 0.988994828981853)
(150, 0.993237573544122)
(160, 0.995851611721499)
(170, 0.997380825782385)
(180, 0.998299868550625)
(190, 0.998882490920958)
(200, 0.999244465392435)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.00244352260748318)
(60, 0.155695932426786)
(70, 0.504199505574439)
(80, 0.745892869601977)
(90, 0.848775377169383)
(100, 0.919188554705237)
(110, 0.950558984178399)
(120, 0.971240081336273)
(130, 0.982199166138003)
(140, 0.988800263411849)
(150, 0.992869181386577)
(160, 0.995221013725292)
(170, 0.996744355063684)
(180, 0.997594848647755)
(190, 0.998298730884705)
(200, 0.998683857946192)
};


==> graphs/B.k10.l005.L25.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.979025924252309)
(60, 0.989609016245936)
(70, 0.994704489052836)
(80, 0.997239755047925)
(90, 0.998498690735024)
(100, 0.99914689616652)
(110, 0.999479951995962)
(120, 0.999672316038774)
(130, 0.999791776155786)
(140, 0.999860203524739)
(150, 0.99990369007697)
(160, 0.999931828434296)
(170, 0.999949350956813)
(180, 0.999962908528979)
(190, 0.99997083842968)
(200, 0.999973908068661)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.00163432695415456)
(60, 0.139179222023023)
(70, 0.511671598766466)
(80, 0.764071768670983)
(90, 0.866432589640813)
(100, 0.937984467370953)
(110, 0.965701388845367)
(120, 0.983118008817282)
(130, 0.991031026503903)
(140, 0.995326858356242)
(150, 0.997484175051791)
(160, 0.998620453081272)
(170, 0.9991784878677)
(180, 0.999517938778353)
(190, 0.999696233642501)
(200, 0.999798682843494)
};
% POLen
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.00158355000934321)
(60, 0.123624593896355)
(70, 0.489015105053918)
(80, 0.755297205643685)
(90, 0.845574136961408)
(100, 0.917756058092406)
(110, 0.948002362087196)
(120, 0.969990314009999)
(130, 0.981375860793919)
(140, 0.988856570990709)
(150, 0.993141914909863)
(160, 0.99578372295792)
(170, 0.997330309397866)
(180, 0.998262840139981)
(190, 0.998853361938958)
(200, 0.999218393174453)
};
% POWork
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(50, 0.00239227197922264)
(60, 0.154078098522365)
(70, 0.501529511573115)
(80, 0.743834022573869)
(90, 0.847501102831755)
(100, 0.918404391425526)
(110, 0.950064647875957)
(120, 0.97092182153912)
(130, 0.981994648851846)
(140, 0.988662032620286)
(150, 0.992773558232139)
(160, 0.995153167950565)
(170, 0.996693870915797)
(180, 0.997557846387335)
(190, 0.998269618926064)
(200, 0.998657800355541)
};


==> graphs/k.B50.l001.L10.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.04)
(2.000000, 0.58)
(3.000000, 1.13)
(4.000000, 1.77)
(5.000000, 2.42)
(6.000000, 3.01)
(7.000000, 3.71)
(8.000000, 4.37)
(9.000000, 5.09)
(10.000000, 5.92)
(11.000000, 7.07)
(12.000000, 7.61)
(13.000000, 8.25)
(14.000000, 9.87)
(15.000000, 10.37)
(16.000000, 11.66)
(17.000000, 13.09)
(18.000000, 17.55)
(19.000000, 16.61)
(20.000000, 19.74)
(21.000000, 17.16)
(22.000000, 22.19)
(23.000000, 27.48)
(24.000000, 23.61)
(25.000000, 44.75)
(26.000000, 39.56)
(27.000000, 48.96)
(28.000000, 37.19)
(29.000000, 50.31)
(30.000000, 50.29)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.04)
(2.000000, 0.58)
(3.000000, 1.12)
(4.000000, 1.74)
(5.000000, 2.37)
(6.000000, 2.95)
(7.000000, 3.60)
(8.000000, 4.22)
(9.000000, 4.91)
(10.000000, 5.71)
(11.000000, 6.77)
(12.000000, 7.29)
(13.000000, 7.89)
(14.000000, 9.40)
(15.000000, 9.86)
(16.000000, 11.08)
(17.000000, 12.37)
(18.000000, 15.84)
(19.000000, 15.04)
(20.000000, 17.48)
(21.000000, 15.99)
(22.000000, 20.12)
(23.000000, 24.25)
(24.000000, 21.83)
(25.000000, 36.81)
(26.000000, 32.95)
(27.000000, 42.17)
(28.000000, 34.61)
(29.000000, 41.44)
(30.000000, 44.11)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.04)
(2.000000, 0.59)
(3.000000, 1.16)
(4.000000, 1.82)
(5.000000, 2.51)
(6.000000, 3.14)
(7.000000, 3.89)
(8.000000, 4.63)
(9.000000, 5.38)
(10.000000, 6.32)
(11.000000, 7.65)
(12.000000, 8.25)
(13.000000, 9.05)
(14.000000, 10.77)
(15.000000, 11.58)
(16.000000, 13.24)
(17.000000, 14.88)
(18.000000, 20.18)
(19.000000, 18.89)
(20.000000, 22.39)
(21.000000, 19.44)
(22.000000, 26.17)
(23.000000, 32.30)
(24.000000, 28.94)
(25.000000, 50.20)
(26.000000, 45.95)
(27.000000, 57.44)
(28.000000, 44.70)
(29.000000, 55.94)
(30.000000, 59.59)
};


==> graphs/k.B50.l001.L10.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.999890464119175)
(3, 1.00000767347816)
(4, 0.999958083229939)
(5, 0.999353350721014)
(6, 0.999731480549122)
(7, 0.999269341376823)
(8, 0.999705610897171)
(9, 0.999148799892125)
(10, 0.998873272412002)
(11, 0.998899356546904)
(12, 0.999657114446626)
(13, 0.999685810654715)
(14, 0.998494024854007)
(15, 0.999855346611773)
(16, 0.999846111569112)
(17, 0.9997243098757)
(18, 0.999430127271576)
(19, 0.99949543791784)
(20, 0.999111985463885)
(21, 0.999586236573377)
(22, 0.999457445137709)
(23, 0.998897672514252)
(24, 1.00001718980988)
(25, 0.998038605230386)
(26, 0.998756605533105)
(27, 0.997085706716121)
(28, 0.999055730084076)
(29, 0.998270013568521)
(30, 0.999081357294597)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.99984352017025)
(3, 1.00000767347816)
(4, 0.999849099627779)
(5, 0.999094691009419)
(6, 0.999739871781962)
(7, 0.998566785008384)
(8, 0.999641959199262)
(9, 0.998676847357066)
(10, 0.998214795250185)
(11, 0.998222037498846)
(12, 0.999408522420429)
(13, 0.999380862172527)
(14, 0.996977215354446)
(15, 0.999298987426282)
(16, 0.999824127507557)
(17, 0.999604444604265)
(18, 0.997889360265096)
(19, 0.998009782898149)
(20, 0.997363279915844)
(21, 0.99892421509078)
(22, 0.99798683590571)
(23, 0.99703946332399)
(24, 0.999879671330835)
(25, 0.990706724782067)
(26, 0.996040770250151)
(27, 0.991273678632931)
(28, 0.995405763678294)
(29, 0.993351424694708)
(30, 0.994641250885151)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.999890464119175)
(3, 1.00000767347816)
(4, 0.999958083229939)
(5, 0.999130615969363)
(6, 0.999647568220723)
(7, 0.998707296282072)
(8, 0.999395308869864)
(9, 0.998314455231931)
(10, 0.997629482217458)
(11, 0.997937255626366)
(12, 0.998928482645705)
(13, 0.999380862172527)
(14, 0.996673853454534)
(15, 0.99942138644709)
(16, 0.999450398461116)
(17, 0.999280808371391)
(18, 0.998184849827983)
(19, 0.997813564310642)
(20, 0.997677500444007)
(21, 0.998874563479585)
(22, 0.998072502462914)
(23, 0.997086705930522)
(24, 0.999793722281432)
(25, 0.991967621419676)
(26, 0.995729921633428)
(27, 0.989816531990992)
(28, 0.993353792514845)
(29, 0.991926729986431)
(30, 0.993913992076707)
};


==> graphs/k.B50.l001.L10.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 0.999992326580724)
(4, 0.999991616716268)
(5, 0.999992815059635)
(6, 0.999991608837572)
(7, 0.999625443615218)
(8, 0.999992043601066)
(9, 0.999865174598894)
(10, 0.999298117346006)
(11, 1)
(12, 1)
(13, 0.999990759222296)
(14, 0.999707558000996)
(15, 0.999988872940103)
(16, 0.999989008090046)
(17, 0.999988013616532)
(18, 0.99941991077173)
(19, 0.996591845571494)
(20, 0.999822428629969)
(21, 0.999371474883806)
(22, 0.998460376067401)
(23, 0.999590731645888)
(24, 0.999982810485604)
(25, 0.996525192355423)
(26, 0.998823433287033)
(27, 0.994368887278954)
(28, 0.990414013884393)
(29, 0.99282659212609)
(30, 0.99476449758215)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.999890464119175)
(3, 1)
(4, 0.999949700297607)
(5, 0.999346170426785)
(6, 0.999723091639885)
(7, 0.998895058664894)
(8, 0.999697656840514)
(9, 0.999014089254415)
(10, 0.998172180588558)
(11, 0.998899356546904)
(12, 0.999657114446626)
(13, 0.999676572780365)
(14, 0.998202023265386)
(15, 0.999844221161443)
(16, 0.999835121350686)
(17, 0.999712326796759)
(18, 0.998850368620337)
(19, 0.99608900311483)
(20, 0.998934571779811)
(21, 0.998957971517888)
(22, 0.997918656535561)
(23, 0.998488855307896)
(24, 1)
(25, 0.994570613055349)
(26, 0.997581501756679)
(27, 0.991471004709059)
(28, 0.989478795726772)
(29, 0.991109015592901)
(30, 0.993850664432852)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.99984352017025)
(3, 1)
(4, 0.999840717609087)
(5, 0.999087512573646)
(6, 0.999731482802313)
(7, 0.998192765443428)
(8, 0.999634005649043)
(9, 0.998542200350546)
(10, 0.997514165600439)
(11, 0.998222037498846)
(12, 0.999408522420429)
(13, 0.999371627116138)
(14, 0.996685657344627)
(15, 0.999287868166594)
(16, 0.999813137530777)
(17, 0.999592462962075)
(18, 0.997310495396201)
(19, 0.994608411436872)
(20, 0.99718617675181)
(21, 0.99829636613242)
(22, 0.996450311488731)
(23, 0.996631406623851)
(24, 0.99986248388483)
(25, 0.987264209481261)
(26, 0.994868861835117)
(27, 0.985691704811144)
(28, 0.985863817848279)
(29, 0.986225709763244)
(30, 0.989433804211248)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.999890464119175)
(3, 1)
(4, 0.999949700297607)
(5, 0.999123437275471)
(6, 0.999639180015608)
(7, 0.998333224087721)
(8, 0.999387357282094)
(9, 0.998179857085075)
(10, 0.996929263388777)
(11, 0.997937255626366)
(12, 0.998928482645705)
(13, 0.999371627116138)
(14, 0.996382384160475)
(15, 0.999410265825461)
(16, 0.999439412592332)
(17, 0.999268830608429)
(18, 0.997605813548775)
(19, 0.994412861592614)
(20, 0.997500341483404)
(21, 0.99824674572851)
(22, 0.996535846151653)
(23, 0.996678629895479)
(24, 0.999776536312849)
(25, 0.988520724745594)
(26, 0.994558378952529)
(27, 0.984242763526196)
(28, 0.983831516851912)
(29, 0.984811234971205)
(30, 0.988710352968054)
};


==> graphs/k.B50.l001.L15.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.02)
(2.000000, 0.57)
(3.000000, 1.10)
(4.000000, 1.76)
(5.000000, 2.26)
(6.000000, 2.80)
(7.000000, 3.36)
(8.000000, 4.13)
(9.000000, 4.85)
(10.000000, 5.65)
(11.000000, 6.46)
(12.000000, 7.16)
(13.000000, 8.32)
(14.000000, 9.45)
(15.000000, 10.09)
(16.000000, 11.61)
(17.000000, 12.84)
(18.000000, 13.44)
(19.000000, 17.72)
(20.000000, 17.97)
(21.000000, 15.73)
(22.000000, 19.98)
(23.000000, 20.85)
(24.000000, 28.44)
(25.000000, 34.40)
(26.000000, 26.31)
(27.000000, 33.66)
(28.000000, 27.76)
(29.000000, 42.85)
(30.000000, 48.46)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.02)
(2.000000, 0.57)
(3.000000, 1.08)
(4.000000, 1.73)
(5.000000, 2.23)
(6.000000, 2.76)
(7.000000, 3.30)
(8.000000, 4.04)
(9.000000, 4.74)
(10.000000, 5.51)
(11.000000, 6.24)
(12.000000, 6.91)
(13.000000, 7.98)
(14.000000, 9.07)
(15.000000, 9.61)
(16.000000, 10.88)
(17.000000, 12.15)
(18.000000, 12.63)
(19.000000, 16.20)
(20.000000, 16.55)
(21.000000, 14.89)
(22.000000, 18.37)
(23.000000, 19.27)
(24.000000, 25.17)
(25.000000, 30.05)
(26.000000, 24.05)
(27.000000, 30.35)
(28.000000, 25.64)
(29.000000, 37.37)
(30.000000, 41.40)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.02)
(2.000000, 0.58)
(3.000000, 1.11)
(4.000000, 1.81)
(5.000000, 2.32)
(6.000000, 2.88)
(7.000000, 3.48)
(8.000000, 4.31)
(9.000000, 5.10)
(10.000000, 5.95)
(11.000000, 6.91)
(12.000000, 7.68)
(13.000000, 9.07)
(14.000000, 10.38)
(15.000000, 10.93)
(16.000000, 12.80)
(17.000000, 14.44)
(18.000000, 15.21)
(19.000000, 20.11)
(20.000000, 20.74)
(21.000000, 17.97)
(22.000000, 22.72)
(23.000000, 24.21)
(24.000000, 33.65)
(25.000000, 41.00)
(26.000000, 30.95)
(27.000000, 40.57)
(28.000000, 33.17)
(29.000000, 52.76)
(30.000000, 57.75)
};


==> graphs/k.B50.l001.L15.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.992781507633691)
(2, 0.979183911053674)
(3, 0.973627815946431)
(4, 0.963808118665802)
(5, 0.968195982926127)
(6, 0.946927591649808)
(7, 0.942963499767996)
(8, 0.953822035492569)
(9, 0.980594311645403)
(10, 0.987539679942403)
(11, 0.98997815551084)
(12, 0.992125263254281)
(13, 0.993699093284156)
(14, 0.99261579552038)
(15, 0.995338997431923)
(16, 0.99781666955467)
(17, 0.996990961265887)
(18, 0.997603753701009)
(19, 0.994925534139818)
(20, 0.996459997977142)
(21, 0.999291341178022)
(22, 0.997541295370572)
(23, 0.996177750155376)
(24, 0.994571296475817)
(25, 0.993540408816469)
(26, 0.997108063976707)
(27, 0.99505193770864)
(28, 0.998822526290146)
(29, 0.99521477137241)
(30, 0.99555242176059)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.99133238172256)
(2, 0.977688655818946)
(3, 0.971728739931122)
(4, 0.961060308249868)
(5, 0.966952104119203)
(6, 0.943159333940997)
(7, 0.938490253223292)
(8, 0.951106791246002)
(9, 0.977044895142939)
(10, 0.984725267532808)
(11, 0.988067741405094)
(12, 0.990522845893233)
(13, 0.991565644238332)
(14, 0.990583175404315)
(15, 0.993121627278178)
(16, 0.995517818979957)
(17, 0.995376071752213)
(18, 0.99618607918904)
(19, 0.989873083315905)
(20, 0.993122281784161)
(21, 0.998582682356043)
(22, 0.994987502716801)
(23, 0.992153511497825)
(24, 0.98781524511193)
(25, 0.984272932276133)
(26, 0.994137435816726)
(27, 0.989883584972803)
(28, 0.997381136059117)
(29, 0.989446718009861)
(30, 0.988555621847372)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.992781507633691)
(2, 0.979525683678755)
(3, 0.974458298729884)
(4, 0.963966550978072)
(5, 0.968333464267945)
(6, 0.947155465641048)
(7, 0.942217958677212)
(8, 0.951182040509187)
(9, 0.977369981888024)
(10, 0.984488006021534)
(11, 0.986713226485856)
(12, 0.988251991575863)
(13, 0.990399479293792)
(14, 0.989021887489076)
(15, 0.991096580045931)
(16, 0.995055738462427)
(17, 0.994051629992797)
(18, 0.995847342801224)
(19, 0.98837606084956)
(20, 0.992992240893525)
(21, 0.997956425722667)
(22, 0.994661486633341)
(23, 0.992308887507769)
(24, 0.988098611504676)
(25, 0.984636647995926)
(26, 0.992386535775413)
(27, 0.988324606442648)
(28, 0.99725932843396)
(29, 0.987819418038862)
(30, 0.988230189293269)
};


==> graphs/k.B50.l001.L15.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 0.99999372926739)
(9, 0.999277370423899)
(10, 0.999991818635512)
(11, 0.999992170495294)
(12, 1)
(13, 0.999990960043392)
(14, 0.999627001187707)
(15, 0.999988687014956)
(16, 0.999988448120509)
(17, 0.999988382224804)
(18, 0.999987454365254)
(19, 0.998834562906116)
(20, 0.999812198434024)
(21, 0.99998351983388)
(22, 0.999416228838295)
(23, 0.999192697012979)
(24, 0.998198654201155)
(25, 0.998561757271116)
(26, 0.994930514777843)
(27, 0.995848731838202)
(28, 0.999979699141274)
(29, 0.99693207189553)
(30, 0.997835146398225)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.992781507633691)
(2, 0.979183911053674)
(3, 0.973627815946431)
(4, 0.963808118665802)
(5, 0.968195982926127)
(6, 0.946927591649808)
(7, 0.942963499767996)
(8, 0.953816054329627)
(9, 0.979885705193651)
(10, 0.987531600520335)
(11, 0.989970404472213)
(12, 0.992125263254281)
(13, 0.993690110287471)
(14, 0.992245551007588)
(15, 0.995327737176731)
(16, 0.997805142896749)
(17, 0.996979378449027)
(18, 0.997591238128693)
(19, 0.993766011016679)
(20, 0.996272861229089)
(21, 0.999274872690717)
(22, 0.996958959529725)
(23, 0.995373532882072)
(24, 0.992779729649259)
(25, 0.992111456547636)
(26, 0.992053239381484)
(27, 0.990921210280295)
(28, 0.998802249335147)
(29, 0.992161524005333)
(30, 0.993397196514586)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.99133238172256)
(2, 0.977688655818946)
(3, 0.971728739931122)
(4, 0.961060308249868)
(5, 0.966952104119203)
(6, 0.943159333940997)
(7, 0.938490253223292)
(8, 0.951100827109631)
(9, 0.976338853604529)
(10, 0.984717211136473)
(11, 0.988060005324063)
(12, 0.990522845893233)
(13, 0.991556680527933)
(14, 0.990213689056411)
(15, 0.993110392108062)
(16, 0.995506318878081)
(17, 0.995364507696776)
(18, 0.996173581402351)
(19, 0.988719448506371)
(20, 0.992935771864436)
(21, 0.998566225547553)
(22, 0.994406657706458)
(23, 0.991352543004409)
(24, 0.986035848270113)
(25, 0.98285730888805)
(26, 0.98909767077706)
(27, 0.985774312762618)
(28, 0.997360888365578)
(29, 0.986411166615802)
(30, 0.986415543648861)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.992781507633691)
(2, 0.979525683678755)
(3, 0.974458298729884)
(4, 0.963966550978072)
(5, 0.968333464267945)
(6, 0.947155465641048)
(7, 0.942217958677212)
(8, 0.951176075900948)
(9, 0.976663705432318)
(10, 0.984479951566322)
(11, 0.986705501010006)
(12, 0.988251991575863)
(13, 0.990390526125475)
(14, 0.98865298349971)
(15, 0.991085367785144)
(16, 0.99504424369845)
(17, 0.994040081324426)
(18, 0.995834849264199)
(19, 0.98722417072554)
(20, 0.992805755395683)
(21, 0.997939979234991)
(22, 0.994080831941786)
(23, 0.991507793578836)
(24, 0.986318704221997)
(25, 0.983220501496354)
(26, 0.987355646897632)
(27, 0.984221805970401)
(28, 0.99723908321322)
(29, 0.984788859084119)
(30, 0.986090815608594)
};


==> graphs/k.B50.l005.L10.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.22)
(2.000000, 1.12)
(3.000000, 2.42)
(4.000000, 4.39)
(5.000000, 7.94)
(6.000000, 17.66)
(7.000000, 35.08)
(8.000000, 46.60)
(9.000000, 45.15)
(10.000000, 43.10)
(11.000000, 42.05)
(12.000000, 40.50)
(13.000000, 40.54)
(14.000000, 40.67)
(15.000000, 40.45)
(16.000000, 41.32)
(17.000000, 42.76)
(18.000000, 42.51)
(19.000000, 43.72)
(20.000000, 44.24)
(21.000000, 44.87)
(22.000000, 45.52)
(23.000000, 45.47)
(24.000000, 46.72)
(25.000000, 46.91)
(26.000000, 48.25)
(27.000000, 48.95)
(28.000000, 49.65)
(29.000000, 50.12)
(30.000000, 51.91)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.22)
(2.000000, 1.05)
(3.000000, 2.21)
(4.000000, 3.91)
(5.000000, 6.72)
(6.000000, 12.63)
(7.000000, 22.02)
(8.000000, 30.87)
(9.000000, 34.89)
(10.000000, 37.18)
(11.000000, 38.84)
(12.000000, 40.08)
(13.000000, 41.74)
(14.000000, 42.51)
(15.000000, 43.63)
(16.000000, 44.99)
(17.000000, 46.37)
(18.000000, 47.09)
(19.000000, 48.46)
(20.000000, 48.91)
(21.000000, 50.28)
(22.000000, 51.46)
(23.000000, 51.98)
(24.000000, 53.48)
(25.000000, 54.37)
(26.000000, 55.67)
(27.000000, 56.53)
(28.000000, 57.27)
(29.000000, 58.07)
(30.000000, 60.10)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.22)
(2.000000, 1.19)
(3.000000, 2.69)
(4.000000, 5.08)
(5.000000, 9.43)
(6.000000, 19.36)
(7.000000, 34.07)
(8.000000, 43.33)
(9.000000, 44.02)
(10.000000, 43.64)
(11.000000, 44.56)
(12.000000, 44.57)
(13.000000, 46.06)
(14.000000, 47.61)
(15.000000, 48.78)
(16.000000, 50.95)
(17.000000, 53.58)
(18.000000, 55.10)
(19.000000, 57.75)
(20.000000, 59.71)
(21.000000, 62.22)
(22.000000, 64.38)
(23.000000, 66.77)
(24.000000, 69.93)
(25.000000, 71.66)
(26.000000, 74.43)
(27.000000, 77.29)
(28.000000, 79.25)
(29.000000, 82.03)
(30.000000, 84.81)
};


==> graphs/k.B50.l005.L10.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
};\label{gr:FOPTUW}
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1.00000015245134)
(4, 0.999986936807413)
(5, 0.99995716011155)
(6, 0.999517980017165)
(7, 0.998365489790958)
(8, 0.99728696102451)
(9, 0.997047173368087)
(10, 0.997099612275403)
(11, 0.997116622814212)
(12, 0.997179734242994)
(13, 0.997337352921326)
(14, 0.997465127881905)
(15, 0.997562504458083)
(16, 0.997732747515723)
(17, 0.997843481700626)
(18, 0.998070419594158)
(19, 0.99810009418682)
(20, 0.998196824820201)
(21, 0.998176361258224)
(22, 0.998292899071938)
(23, 0.998386324682515)
(24, 0.998411453114359)
(25, 0.998454722409015)
(26, 0.998436648169722)
(27, 0.998428331672179)
(28, 0.998458951731277)
(29, 0.998434112199938)
(30, 0.998434887480379)
};\label{gr:POValue}
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.999998465972744)
(3, 0.999993292140981)
(4, 0.999850532773196)
(5, 0.999400088013706)
(6, 0.993494791451161)
(7, 0.978695004861449)
(8, 0.953645135420124)
(9, 0.933270803135289)
(10, 0.914097010674193)
(11, 0.905072174149008)
(12, 0.892924082585661)
(13, 0.889335643096583)
(14, 0.885600861359268)
(15, 0.882259864686171)
(16, 0.880203333705217)
(17, 0.88152599613829)
(18, 0.879265721549809)
(19, 0.879577672000516)
(20, 0.880115771674213)
(21, 0.879737852209305)
(22, 0.880284011554777)
(23, 0.879944166603983)
(24, 0.880478587147825)
(25, 0.879305082323437)
(26, 0.880880053894367)
(27, 0.880147875462363)
(28, 0.881124980489038)
(29, 0.881134716413797)
(30, 0.881949568774312)
};\label{gr:POWork}
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 0.999996188716466)
(4, 0.999952607952477)
(5, 0.999776434130524)
(6, 0.997659218132135)
(7, 0.992250091152163)
(8, 0.984245705540858)
(9, 0.976117336871998)
(10, 0.966230307436879)
(11, 0.958079389447886)
(12, 0.943507575734054)
(13, 0.935374564107179)
(14, 0.923893906454647)
(15, 0.910501172771569)
(16, 0.900681094056786)
(17, 0.893646898717911)
(18, 0.878199201067221)
(19, 0.86921286668129)
(20, 0.856095635965766)
(21, 0.847548523447357)
(22, 0.838297729542069)
(23, 0.824499165558487)
(24, 0.816615678031703)
(25, 0.805799060768071)
(26, 0.799418450912581)
(27, 0.790902573704565)
(28, 0.779004221485904)
(29, 0.7681177708653)
(30, 0.76270861768921)
};\label{gr:POLen}


==> graphs/k.B50.l005.L10.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 0.999999847548682)
(4, 0.999953977148971)
(5, 0.999995393581601)
(6, 0.999489536334178)
(7, 0.995390361511008)
(8, 0.981321412112657)
(9, 0.95945105792988)
(10, 0.93057918740925)
(11, 0.909013675577725)
(12, 0.871599438611473)
(13, 0.852749995472362)
(14, 0.826176238083026)
(15, 0.795734807005806)
(16, 0.774150800985596)
(17, 0.763007954877851)
(18, 0.732940417530396)
(19, 0.718541628480111)
(20, 0.696784178490245)
(21, 0.685093931192664)
(22, 0.671775328869682)
(23, 0.646998188287973)
(24, 0.640848280995971)
(25, 0.622495131870538)
(26, 0.618861884261381)
(27, 0.607550702582371)
(28, 0.593321418697391)
(29, 0.580898480925524)
(30, 0.580167571368938)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 0.99994091455759)
(5, 0.999952553890489)
(6, 0.99900776240503)
(7, 0.993763385803136)
(8, 0.978659048874112)
(9, 0.956617965294008)
(10, 0.927880146957323)
(11, 0.906392646283995)
(12, 0.869141296560932)
(13, 0.850479423188077)
(14, 0.824081986972477)
(15, 0.793795206961181)
(16, 0.772395605658856)
(17, 0.761362514260589)
(18, 0.73152615006208)
(19, 0.71717646706315)
(20, 0.695527754553915)
(21, 0.683844567357985)
(22, 0.670628540582319)
(23, 0.645954143281075)
(24, 0.639830263455027)
(25, 0.621533204092761)
(26, 0.617894385401932)
(27, 0.606595834385577)
(28, 0.592407081752311)
(29, 0.579988859081168)
(30, 0.57925954383951)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.999998465972744)
(3, 0.999993139690685)
(4, 0.999804516801075)
(5, 0.999395484358753)
(6, 0.992987648457942)
(7, 0.974183574698055)
(8, 0.935832390944842)
(9, 0.895427659403222)
(10, 0.850639653406415)
(11, 0.822722983686312)
(12, 0.778272129104327)
(13, 0.758380965624021)
(14, 0.731662388080888)
(15, 0.702044883155018)
(16, 0.681410115818085)
(17, 0.672611347485137)
(18, 0.644449385072882)
(19, 0.632013172813995)
(20, 0.613250744942325)
(21, 0.602703063589064)
(22, 0.591353081360933)
(23, 0.569322281587347)
(24, 0.564253189027445)
(25, 0.547363133175362)
(26, 0.545143089961335)
(27, 0.53473446011354)
(28, 0.522790323473467)
(29, 0.511849818255517)
(30, 0.511678539385675)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 0.999996036265729)
(4, 0.999906587282565)
(5, 0.999771828741963)
(6, 0.997149949350406)
(7, 0.987676176941283)
(8, 0.965861385627173)
(9, 0.936536811525536)
(10, 0.899153814344801)
(11, 0.870907267297285)
(12, 0.822360673335473)
(13, 0.797640655307359)
(14, 0.763299192022531)
(15, 0.724517474993944)
(16, 0.697262990396643)
(17, 0.681859692573688)
(18, 0.643667689105069)
(19, 0.624565628721039)
(20, 0.59651389441549)
(21, 0.580650349805087)
(22, 0.563147732953831)
(23, 0.532155469984711)
(24, 0.523326753500976)
(25, 0.500361002330235)
(26, 0.494729608845075)
(27, 0.480513414328414)
(28, 0.462199889863273)
(29, 0.446198446267552)
(30, 0.445399644243754)
};


==> graphs/k.B50.l005.L15.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.22)
(2.000000, 1.12)
(3.000000, 2.35)
(4.000000, 4.39)
(5.000000, 7.46)
(6.000000, 12.54)
(7.000000, 17.61)
(8.000000, 20.68)
(9.000000, 22.00)
(10.000000, 22.39)
(11.000000, 22.09)
(12.000000, 22.23)
(13.000000, 22.34)
(14.000000, 22.62)
(15.000000, 22.95)
(16.000000, 23.63)
(17.000000, 23.76)
(18.000000, 24.29)
(19.000000, 24.63)
(20.000000, 25.05)
(21.000000, 25.50)
(22.000000, 26.08)
(23.000000, 26.50)
(24.000000, 26.97)
(25.000000, 27.42)
(26.000000, 28.01)
(27.000000, 28.64)
(28.000000, 29.11)
(29.000000, 29.90)
(30.000000, 29.76)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.22)
(2.000000, 1.05)
(3.000000, 2.14)
(4.000000, 3.84)
(5.000000, 6.15)
(6.000000, 9.57)
(7.000000, 13.30)
(8.000000, 16.56)
(9.000000, 18.95)
(10.000000, 20.87)
(11.000000, 21.99)
(12.000000, 23.29)
(13.000000, 24.25)
(14.000000, 25.11)
(15.000000, 26.08)
(16.000000, 26.92)
(17.000000, 27.64)
(18.000000, 28.44)
(19.000000, 28.93)
(20.000000, 29.51)
(21.000000, 30.13)
(22.000000, 30.89)
(23.000000, 31.59)
(24.000000, 31.86)
(25.000000, 32.43)
(26.000000, 33.07)
(27.000000, 34.08)
(28.000000, 34.65)
(29.000000, 35.54)
(30.000000, 35.21)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.22)
(2.000000, 1.19)
(3.000000, 2.58)
(4.000000, 4.93)
(5.000000, 8.30)
(6.000000, 13.13)
(7.000000, 17.57)
(8.000000, 20.69)
(9.000000, 22.30)
(10.000000, 23.34)
(11.000000, 23.83)
(12.000000, 24.62)
(13.000000, 25.30)
(14.000000, 26.17)
(15.000000, 27.08)
(16.000000, 28.22)
(17.000000, 29.07)
(18.000000, 30.26)
(19.000000, 31.27)
(20.000000, 32.41)
(21.000000, 33.38)
(22.000000, 34.55)
(23.000000, 35.64)
(24.000000, 37.02)
(25.000000, 37.99)
(26.000000, 39.28)
(27.000000, 40.82)
(28.000000, 41.91)
(29.000000, 43.27)
(30.000000, 44.28)
};


==> graphs/k.B50.l005.L15.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999998236107034)
(2, 0.999978091541544)
(3, 0.999890213216369)
(4, 0.999376892177129)
(5, 0.997989534203345)
(6, 0.994117617391102)
(7, 0.988627191024875)
(8, 0.984706368860064)
(9, 0.983876141659286)
(10, 0.983815705257433)
(11, 0.983948222019869)
(12, 0.984640210503577)
(13, 0.984961728077038)
(14, 0.985836603188551)
(15, 0.986629144946843)
(16, 0.986659115060719)
(17, 0.987850891001999)
(18, 0.988126679834761)
(19, 0.988462392800668)
(20, 0.988837320227151)
(21, 0.988981405522196)
(22, 0.98956712604103)
(23, 0.989866659977784)
(24, 0.989766757169235)
(25, 0.989993124405393)
(26, 0.990179794172854)
(27, 0.990173224441274)
(28, 0.990289661131248)
(29, 0.990324606380775)
(30, 0.990366162592284)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999982361070343)
(2, 0.999879503478494)
(3, 0.999534337919674)
(4, 0.997564102126845)
(5, 0.991908010085124)
(6, 0.977028137962921)
(7, 0.955325656703618)
(8, 0.933334981312544)
(9, 0.918245119494343)
(10, 0.90323916449973)
(11, 0.891298131986948)
(12, 0.883257874750276)
(13, 0.87635609478116)
(14, 0.871963074623399)
(15, 0.86968561262725)
(16, 0.868810776269741)
(17, 0.866911021285678)
(18, 0.86744783396032)
(19, 0.865801068043329)
(20, 0.86657880565081)
(21, 0.866546706551172)
(22, 0.86661633454445)
(23, 0.866668868071152)
(24, 0.867019022330084)
(25, 0.867325591556704)
(26, 0.868141110208838)
(27, 0.867539106353152)
(28, 0.868685197673438)
(29, 0.86820499706512)
(30, 0.868637105009348)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999998236107034)
(2, 0.999936697194559)
(3, 0.999646041446374)
(4, 0.998075796741381)
(5, 0.994636024948374)
(6, 0.985611887703412)
(7, 0.972762608160338)
(8, 0.961152591073721)
(9, 0.952728843084472)
(10, 0.943750398551079)
(11, 0.933385899615541)
(12, 0.923499683963289)
(13, 0.912156689899703)
(14, 0.903003595578247)
(15, 0.893263819483369)
(16, 0.883506107656647)
(17, 0.870578401977961)
(18, 0.862547756140238)
(19, 0.850082489205166)
(20, 0.840288725180264)
(21, 0.831331976066251)
(22, 0.823500028280569)
(23, 0.811943116766463)
(24, 0.7999013873419)
(25, 0.79237056322167)
(26, 0.784778975858878)
(27, 0.777979802828999)
(28, 0.769169722386131)
(29, 0.764776186612343)
(30, 0.748464987766)
};


==> graphs/k.B50.l005.L15.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 0.999980300528744)
(4, 0.999987287893858)
(5, 0.999844973660049)
(6, 0.998577286139908)
(7, 0.992630832387452)
(8, 0.977748369112927)
(9, 0.960414083828027)
(10, 0.934968778233343)
(11, 0.905909056631915)
(12, 0.879660622005626)
(13, 0.853108895277331)
(14, 0.826846011981941)
(15, 0.80366869246157)
(16, 0.785738723886477)
(17, 0.757624232454142)
(18, 0.742802261509771)
(19, 0.721231791882594)
(20, 0.702166453160504)
(21, 0.68970827894408)
(22, 0.676956152595361)
(23, 0.658408954265363)
(24, 0.642478575942924)
(25, 0.631683199459735)
(26, 0.621556686911818)
(27, 0.612675960967744)
(28, 0.603008561852368)
(29, 0.59684410334185)
(30, 0.575826737105388)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999998236107034)
(2, 0.999978091541544)
(3, 0.999870515907855)
(4, 0.999364187992)
(5, 0.997834819538549)
(6, 0.992703272478278)
(7, 0.98134183154789)
(8, 0.96279504620804)
(9, 0.944928503191957)
(10, 0.919836967951317)
(11, 0.891367605584669)
(12, 0.866149220023327)
(13, 0.840279611730253)
(14, 0.815135063812277)
(15, 0.792922954863906)
(16, 0.77525627397877)
(17, 0.74841977307453)
(18, 0.733982732439402)
(19, 0.712910502768182)
(20, 0.694328393896636)
(21, 0.682108663110411)
(22, 0.669893554379584)
(23, 0.651737072458121)
(24, 0.635903936661736)
(25, 0.625362024267539)
(26, 0.615452872313105)
(27, 0.606655331809088)
(28, 0.597153144376023)
(29, 0.591069401712704)
(30, 0.570279315945099)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999982361070343)
(2, 0.999879503478494)
(3, 0.999514647621715)
(4, 0.997551420986096)
(5, 0.991754238216753)
(6, 0.975638106489341)
(7, 0.948285701814802)
(8, 0.912566755814385)
(9, 0.881895545168717)
(10, 0.844500418084818)
(11, 0.807435049926084)
(12, 0.776967171494195)
(13, 0.747627179888311)
(14, 0.720979190847869)
(15, 0.698939099152782)
(16, 0.682658270645006)
(17, 0.656792797107598)
(18, 0.644342212807478)
(19, 0.624443255718754)
(20, 0.608482566347895)
(21, 0.59766443760007)
(22, 0.586661259609505)
(23, 0.570622543121074)
(24, 0.557041146782058)
(25, 0.547875004647846)
(26, 0.539598912233353)
(27, 0.531520355662015)
(28, 0.5238246117515)
(29, 0.518183032990245)
(30, 0.500184469906203)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999998236107034)
(2, 0.999936697194559)
(3, 0.999626348947915)
(4, 0.998063109095915)
(5, 0.994481830165843)
(6, 0.984209644010104)
(7, 0.965594157453585)
(8, 0.939765378390995)
(9, 0.915014198967509)
(10, 0.882377157090533)
(11, 0.845562739794246)
(12, 0.812366306417145)
(13, 0.778168986040163)
(14, 0.746644921809227)
(15, 0.717888165827427)
(16, 0.694204961576042)
(17, 0.659571293589707)
(18, 0.640702423921147)
(19, 0.613106516937458)
(20, 0.590022553790587)
(21, 0.573376546443836)
(22, 0.557473410806985)
(23, 0.534590618433167)
(24, 0.513919504234193)
(25, 0.500527172533577)
(26, 0.487784620192894)
(27, 0.476649523311753)
(28, 0.463815928116445)
(29, 0.456452157355843)
(30, 0.43098615174292)
};


==> graphs/k.B50.l005.L25.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.09)
(2.000000, 0.71)
(3.000000, 1.39)
(4.000000, 2.14)
(5.000000, 2.92)
(6.000000, 3.81)
(7.000000, 4.67)
(8.000000, 5.62)
(9.000000, 6.51)
(10.000000, 7.51)
(11.000000, 8.52)
(12.000000, 9.47)
(13.000000, 10.40)
(14.000000, 11.22)
(15.000000, 11.97)
(16.000000, 12.73)
(17.000000, 13.49)
(18.000000, 14.07)
(19.000000, 14.52)
(20.000000, 15.14)
(21.000000, 15.76)
(22.000000, 16.13)
(23.000000, 16.55)
(24.000000, 16.91)
(25.000000, 17.22)
(26.000000, 17.69)
(27.000000, 17.93)
(28.000000, 18.54)
(29.000000, 18.64)
(30.000000, 19.28)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.09)
(2.000000, 0.69)
(3.000000, 1.34)
(4.000000, 2.04)
(5.000000, 2.77)
(6.000000, 3.58)
(7.000000, 4.39)
(8.000000, 5.25)
(9.000000, 6.07)
(10.000000, 7.02)
(11.000000, 7.95)
(12.000000, 8.89)
(13.000000, 9.86)
(14.000000, 10.73)
(15.000000, 11.54)
(16.000000, 12.40)
(17.000000, 13.26)
(18.000000, 14.04)
(19.000000, 14.72)
(20.000000, 15.54)
(21.000000, 16.26)
(22.000000, 16.79)
(23.000000, 17.43)
(24.000000, 18.03)
(25.000000, 18.57)
(26.000000, 19.19)
(27.000000, 19.61)
(28.000000, 20.30)
(29.000000, 20.68)
(30.000000, 21.30)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1.000000, 0.09)
(2.000000, 0.73)
(3.000000, 1.45)
(4.000000, 2.25)
(5.000000, 3.10)
(6.000000, 4.08)
(7.000000, 5.02)
(8.000000, 6.07)
(9.000000, 7.05)
(10.000000, 8.16)
(11.000000, 9.26)
(12.000000, 10.34)
(13.000000, 11.38)
(14.000000, 12.26)
(15.000000, 13.17)
(16.000000, 14.02)
(17.000000, 14.89)
(18.000000, 15.65)
(19.000000, 16.22)
(20.000000, 16.96)
(21.000000, 17.66)
(22.000000, 18.16)
(23.000000, 18.81)
(24.000000, 19.20)
(25.000000, 19.78)
(26.000000, 20.44)
(27.000000, 20.86)
(28.000000, 21.50)
(29.000000, 21.86)
(30.000000, 22.65)
};


==> graphs/k.B50.l005.L25.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999021899354979)
(2, 0.997056688296699)
(3, 0.993412894068919)
(4, 0.988823855083419)
(5, 0.982598813181108)
(6, 0.97481334291601)
(7, 0.967333674195746)
(8, 0.957651194812801)
(9, 0.952095620929043)
(10, 0.939446855406448)
(11, 0.929301116590557)
(12, 0.91699062801766)
(13, 0.905804714150601)
(14, 0.89695182580461)
(15, 0.891051525506227)
(16, 0.883527712436879)
(17, 0.878868192496744)
(18, 0.87345036332607)
(19, 0.866800883849638)
(20, 0.865325725252318)
(21, 0.864817133198462)
(22, 0.863126697873037)
(23, 0.86053889804866)
(24, 0.862004644754627)
(25, 0.860649052224338)
(26, 0.861686102255826)
(27, 0.859662709434449)
(28, 0.860783891012266)
(29, 0.861772739335781)
(30, 0.861846538296349)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.99839055562562)
(2, 0.995984777998314)
(3, 0.991266886983598)
(4, 0.985062362636159)
(5, 0.9777052770419)
(6, 0.966599529510736)
(7, 0.957489624564215)
(8, 0.94455860516973)
(9, 0.937266274807767)
(10, 0.920584720372191)
(11, 0.906653842682242)
(12, 0.891012376116108)
(13, 0.875277910815023)
(14, 0.862430118026294)
(15, 0.855690432574828)
(16, 0.844166372445849)
(17, 0.837923380500324)
(18, 0.827974765743235)
(19, 0.818398253746878)
(20, 0.814370774002296)
(21, 0.811742429107251)
(22, 0.807720519760685)
(23, 0.801729418609779)
(24, 0.801760972888186)
(25, 0.798061132556526)
(26, 0.797540087998573)
(27, 0.793525483164121)
(28, 0.79361986804911)
(29, 0.793752989519947)
(30, 0.792348309515076)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999021899354979)
(2, 0.996429969664398)
(3, 0.991600034899963)
(4, 0.985443780366249)
(5, 0.977618443062802)
(6, 0.966563842126633)
(7, 0.956572474675331)
(8, 0.944036211742099)
(9, 0.936620413308912)
(10, 0.919574657207714)
(11, 0.90526184380734)
(12, 0.888834841783059)
(13, 0.87351512316692)
(14, 0.859767619296643)
(15, 0.85112611531163)
(16, 0.840027944605449)
(17, 0.833548749732421)
(18, 0.8206052035592)
(19, 0.808799357151522)
(20, 0.804159084288627)
(21, 0.799957729310117)
(22, 0.793787446119505)
(23, 0.783871610193)
(24, 0.781813630853011)
(25, 0.774854065586593)
(26, 0.771092822084509)
(27, 0.764542572062218)
(28, 0.764372236719321)
(29, 0.759369615439114)
(30, 0.757550105646313)
};


==> graphs/k.B50.l005.L25.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 0.999998558937554)
(4, 0.999996393225963)
(5, 0.999973515678982)
(6, 0.999832894130178)
(7, 0.999907621640981)
(8, 0.999765896170136)
(9, 0.999236930091689)
(10, 0.998961688298698)
(11, 0.998027980753361)
(12, 0.99695568465449)
(13, 0.994133067805927)
(14, 0.988060009521717)
(15, 0.983288210618088)
(16, 0.979131414951564)
(17, 0.975948911741277)
(18, 0.958817725371744)
(19, 0.946620589320895)
(20, 0.939404233662875)
(21, 0.929109353576699)
(22, 0.917264264340067)
(23, 0.897094813692343)
(24, 0.885993662479192)
(25, 0.871074707246244)
(26, 0.859756707796276)
(27, 0.845890124848329)
(28, 0.844264249222632)
(29, 0.826777172963282)
(30, 0.821350188261255)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999021899354979)
(2, 0.997056688296699)
(3, 0.993411462498904)
(4, 0.988820288619211)
(5, 0.982572789718708)
(6, 0.974650445884428)
(7, 0.9672443134983)
(8, 0.957427005000422)
(9, 0.951369105410877)
(10, 0.938471416743728)
(11, 0.927468516902717)
(12, 0.914199019377097)
(13, 0.900490419311608)
(14, 0.886242229545024)
(15, 0.876160460083536)
(16, 0.865089739227239)
(17, 0.85773045603122)
(18, 0.837479690589426)
(19, 0.820531563493617)
(20, 0.812890649799425)
(21, 0.803509687588077)
(22, 0.791715275556783)
(23, 0.771984982419977)
(24, 0.763730652280227)
(25, 0.749689621208072)
(26, 0.740840406429274)
(27, 0.727180196610959)
(28, 0.726729065488406)
(29, 0.71249402916486)
(30, 0.707877816482017)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.99839055562562)
(2, 0.995984777998314)
(3, 0.991265458506113)
(4, 0.985058809738805)
(5, 0.977679383181481)
(6, 0.966438005055587)
(7, 0.95740117324392)
(8, 0.944337480382728)
(9, 0.936551075117386)
(10, 0.919628866484989)
(11, 0.904865903854433)
(12, 0.888299853466459)
(13, 0.870142714661302)
(14, 0.852132710628875)
(15, 0.841390314289521)
(16, 0.826549814707433)
(17, 0.817770411321863)
(18, 0.793876881555132)
(19, 0.774712637261061)
(20, 0.76502335286907)
(21, 0.754197483578617)
(22, 0.740893168350662)
(23, 0.71922730341941)
(24, 0.710355140802084)
(25, 0.695170867406282)
(26, 0.685690440393205)
(27, 0.671235370024029)
(28, 0.670024882066646)
(29, 0.656256852706455)
(30, 0.650795433188695)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.999021899354979)
(2, 0.996429969664398)
(3, 0.991598605942391)
(4, 0.985440226093207)
(5, 0.977592551502122)
(6, 0.966402323635056)
(7, 0.956484108079838)
(8, 0.9438152092494)
(9, 0.935905706456006)
(10, 0.918619852080915)
(11, 0.903476650028104)
(12, 0.886128948234596)
(13, 0.868390269168802)
(14, 0.849502002108705)
(15, 0.836902274935097)
(16, 0.822497750000387)
(17, 0.813500995184659)
(18, 0.786810814704849)
(19, 0.765626124109135)
(20, 0.755430448319197)
(21, 0.743248208768006)
(22, 0.728112857807188)
(23, 0.703207156104807)
(24, 0.692681922175615)
(25, 0.674955778339403)
(26, 0.662952226120717)
(27, 0.646719011733572)
(28, 0.645332152560461)
(29, 0.627829463886965)
(30, 0.622213921889933)
};


==> graphs/lambda.k10.B50.L10.2.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 1)
(0.01, 1)
(0.015, 1)
(0.02, 1)
(0.025, 1)
(0.03, 1)
(0.035, 1)
(0.04, 1)
(0.045, 1)
(0.05, 1)
(0.055, 1)
(0.06, 1)
(0.065, 1)
(0.07, 1)
(0.075, 1)
(0.08, 1)
(0.085, 1)
(0.09, 1)
(0.095, 1)
(0.1, 1)
(0.105, 1)
(0.11, 1)
(0.115, 1)
(0.12, 1)
(0.125, 1)
(0.13, 1)
(0.135, 1)
(0.14, 1)
(0.145, 1)
(0.15, 1)
(0.155, 1)
(0.16, 1)
(0.165, 1)
(0.17, 1)
(0.175, 1)
(0.18, 1)
(0.185, 1)
(0.19, 1)
(0.195, 1)
(0.2, 1)
(0.205, 1)
(0.21, 1)
(0.215, 1)
(0.22, 1)
(0.225, 1)
(0.23, 1)
(0.235, 1)
(0.24, 1)
(0.245, 1)
(0.25, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 0.999395108553492)
(0.01, 0.999861612977627)
(0.015, 0.99224674890985)
(0.02, 0.987158285580429)
(0.025, 0.984493988787712)
(0.03, 0.966376348342888)
(0.035, 0.959430948083542)
(0.04, 0.950161379898745)
(0.045, 0.938881806849842)
(0.05, 0.937239254134139)
(0.055, 0.936000613991327)
(0.06, 0.936287535031182)
(0.065, 0.937336507491948)
(0.07, 0.937618392713496)
(0.075, 0.936470660241041)
(0.08, 0.939284229468132)
(0.085, 0.937712527265917)
(0.09, 0.937973698770467)
(0.095, 0.93994529326445)
(0.1, 0.939579548285736)
(0.105, 0.940613763840952)
(0.11, 0.942093442413673)
(0.115, 0.94143768052062)
(0.12, 0.941330710208852)
(0.125, 0.9405141161126)
(0.13, 0.940528784477229)
(0.135, 0.940730507612365)
(0.14, 0.939865760434005)
(0.145, 0.940555859480164)
(0.15, 0.939714923721482)
(0.155, 0.939063374200714)
(0.16, 0.938276952082154)
(0.165, 0.937916168398552)
(0.17, 0.938257555214345)
(0.175, 0.939134100541734)
(0.18, 0.938294290912166)
(0.185, 0.938086645232316)
(0.19, 0.937049759857923)
(0.195, 0.937409012453683)
(0.2, 0.936587175349274)
(0.205, 0.93708307294614)
(0.21, 0.93493129901939)
(0.215, 0.935771493132104)
(0.22, 0.936315241970524)
(0.225, 0.935180107988701)
(0.23, 0.934490829324028)
(0.235, 0.935227306260454)
(0.24, 0.93351684532925)
(0.245, 0.934721959089881)
(0.25, 0.934133740682159)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 0.999346063301072)
(0.01, 0.999669408779888)
(0.015, 0.988471757742362)
(0.02, 0.979966505955856)
(0.025, 0.975663501733692)
(0.03, 0.945237850862402)
(0.035, 0.93024293449625)
(0.04, 0.91225118922095)
(0.045, 0.886106098753836)
(0.05, 0.87263378655267)
(0.055, 0.865281092904563)
(0.06, 0.86180416452808)
(0.065, 0.85369556084582)
(0.07, 0.851085013309151)
(0.075, 0.847498716027963)
(0.08, 0.844766428716751)
(0.085, 0.840261507991882)
(0.09, 0.840108771022742)
(0.095, 0.83754206318246)
(0.1, 0.836753290929424)
(0.105, 0.834518367568682)
(0.11, 0.833864165983292)
(0.115, 0.833792824311982)
(0.12, 0.833256089884051)
(0.125, 0.83165829661809)
(0.13, 0.830188622514432)
(0.135, 0.829884080302507)
(0.14, 0.8288175821466)
(0.145, 0.828987317880763)
(0.15, 0.826152338166995)
(0.155, 0.825599847628675)
(0.16, 0.825398587450842)
(0.165, 0.823345892543506)
(0.17, 0.824998910871987)
(0.175, 0.823696873966866)
(0.18, 0.825030444458586)
(0.185, 0.823576756514181)
(0.19, 0.819837575409317)
(0.195, 0.82242270914047)
(0.2, 0.819650399388601)
(0.205, 0.819523380719702)
(0.21, 0.819493746475135)
(0.215, 0.817010951728871)
(0.22, 0.819104872394206)
(0.225, 0.816896944765419)
(0.23, 0.815256064227856)
(0.235, 0.816374344391)
(0.24, 0.813804747320061)
(0.245, 0.814717314379656)
(0.25, 0.814500595303906)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 0.999182579126341)
(0.01, 0.999500269085877)
(0.015, 0.988113617554677)
(0.02, 0.978400187398827)
(0.025, 0.973767782494572)
(0.03, 0.945511551639028)
(0.035, 0.933471597852042)
(0.04, 0.916323918835167)
(0.045, 0.890340020269149)
(0.05, 0.875905071617662)
(0.055, 0.867542115967612)
(0.06, 0.863625558871311)
(0.065, 0.850075619661112)
(0.07, 0.842752624613666)
(0.075, 0.837101868877848)
(0.08, 0.824202652958325)
(0.085, 0.813501127358456)
(0.09, 0.808657709526766)
(0.095, 0.796299018728317)
(0.1, 0.790109748841591)
(0.105, 0.780832048144949)
(0.11, 0.77422122306439)
(0.115, 0.764874475258477)
(0.12, 0.76388306497803)
(0.125, 0.752546446067104)
(0.13, 0.742850986209108)
(0.135, 0.735711748516934)
(0.14, 0.729558712471488)
(0.145, 0.726940186040184)
(0.15, 0.719373734076606)
(0.155, 0.709248225157934)
(0.16, 0.704132643497852)
(0.165, 0.700484014717796)
(0.17, 0.693101507619895)
(0.175, 0.687599596279756)
(0.18, 0.68678340020799)
(0.185, 0.680002642826314)
(0.19, 0.672197873375355)
(0.195, 0.671745643575393)
(0.2, 0.663086921565494)
(0.205, 0.661328524166392)
(0.21, 0.654729529082107)
(0.215, 0.654591600545159)
(0.22, 0.646763313215374)
(0.225, 0.640582602413154)
(0.23, 0.63829276485768)
(0.235, 0.638938631736057)
(0.24, 0.631125574272588)
(0.245, 0.631236745769341)
(0.25, 0.621188155896668)
};


==> graphs/lambda.k10.B50.L10.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 12.44)
(0.050000, 42.82)
(0.075000, 26.90)
(0.100000, 24.27)
(0.125000, 20.72)
(0.150000, 17.89)
(0.175000, 16.66)
(0.200000, 15.94)
(0.225000, 15.19)
(0.250000, 14.46)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 10.80)
(0.050000, 37.08)
(0.075000, 30.09)
(0.100000, 25.84)
(0.125000, 23.01)
(0.150000, 21.44)
(0.175000, 19.39)
(0.200000, 18.00)
(0.225000, 17.98)
(0.250000, 17.19)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 14.83)
(0.050000, 43.72)
(0.075000, 32.46)
(0.100000, 29.88)
(0.125000, 29.18)
(0.150000, 28.75)
(0.175000, 28.43)
(0.200000, 28.30)
(0.225000, 28.71)
(0.250000, 29.16)
};


==> graphs/lambda.k10.B50.L10.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 1)
(0.05, 1)
(0.075, 1)
(0.1, 1)
(0.125, 1)
(0.15, 1)
(0.175, 1)
(0.2, 1)
(0.225, 1)
(0.25, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.999972753511736)
(0.05, 0.997083271763011)
(0.075, 0.997336135072038)
(0.1, 0.997864987264719)
(0.125, 0.998083229638343)
(0.15, 0.997769602625955)
(0.175, 0.997807311989834)
(0.2, 0.997819035170714)
(0.225, 0.997756596267118)
(0.25, 0.997704071641622)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.999603854429054)
(0.05, 0.915049031627389)
(0.075, 0.878563494527304)
(0.1, 0.877228897478307)
(0.125, 0.87526889389732)
(0.15, 0.8729082130557)
(0.175, 0.871359077761194)
(0.2, 0.870794834340176)
(0.225, 0.868688985598119)
(0.25, 0.867145645797303)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.999789681601824)
(0.05, 0.966211452242269)
(0.075, 0.911469013263825)
(0.1, 0.860128589723896)
(0.125, 0.812429275335935)
(0.15, 0.769287234987074)
(0.175, 0.729854927309861)
(0.2, 0.70049984666879)
(0.225, 0.670499109348287)
(0.25, 0.644177336631818)
};


==> graphs/lambda.k10.B50.L15.2.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 1)
(0.01, 1)
(0.015, 1)
(0.02, 1)
(0.025, 1)
(0.03, 1)
(0.035, 1)
(0.04, 1)
(0.045, 1)
(0.05, 1)
(0.055, 1)
(0.06, 1)
(0.065, 1)
(0.07, 1)
(0.075, 1)
(0.08, 1)
(0.085, 1)
(0.09, 1)
(0.095, 1)
(0.1, 1)
(0.105, 1)
(0.11, 1)
(0.115, 1)
(0.12, 1)
(0.125, 1)
(0.13, 1)
(0.135, 1)
(0.14, 1)
(0.145, 1)
(0.15, 1)
(0.155, 1)
(0.16, 1)
(0.165, 1)
(0.17, 1)
(0.175, 1)
(0.18, 1)
(0.185, 1)
(0.19, 1)
(0.195, 1)
(0.2, 1)
(0.205, 1)
(0.21, 1)
(0.215, 1)
(0.22, 1)
(0.225, 1)
(0.23, 1)
(0.235, 1)
(0.24, 1)
(0.245, 1)
(0.25, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 0.994002679006332)
(0.01, 0.98589041314659)
(0.015, 0.968885436031187)
(0.02, 0.951688625253368)
(0.025, 0.923716424482607)
(0.03, 0.909717627305704)
(0.035, 0.888145324083857)
(0.04, 0.867027539993028)
(0.045, 0.858832362431975)
(0.05, 0.851816218962342)
(0.055, 0.848171966579756)
(0.06, 0.848688597055349)
(0.065, 0.847486814278436)
(0.07, 0.852569818170238)
(0.075, 0.850355828026779)
(0.08, 0.850295621674807)
(0.085, 0.853304025749506)
(0.09, 0.851974325217085)
(0.095, 0.855348824318738)
(0.1, 0.856754200524349)
(0.105, 0.853531424752094)
(0.11, 0.856609041335931)
(0.115, 0.857150030651806)
(0.12, 0.855394309540256)
(0.125, 0.856755818691241)
(0.13, 0.85636040683977)
(0.135, 0.857917675261308)
(0.14, 0.859672424451656)
(0.145, 0.860007136099576)
(0.15, 0.859090077510118)
(0.155, 0.857719349412751)
(0.16, 0.857400403497953)
(0.165, 0.858743189392482)
(0.17, 0.858084470361065)
(0.175, 0.85857759832358)
(0.18, 0.858041442473603)
(0.185, 0.858179495762636)
(0.19, 0.856181583619666)
(0.195, 0.858510465278377)
(0.2, 0.858582005011195)
(0.205, 0.857762379058254)
(0.21, 0.856870089396755)
(0.215, 0.856134150680943)
(0.22, 0.856862906178143)
(0.225, 0.855859064174545)
(0.23, 0.857906108819485)
(0.235, 0.856839402427638)
(0.24, 0.855172922799726)
(0.245, 0.855108861733801)
(0.25, 0.85586608468894)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 0.993135046273746)
(0.01, 0.983239375888337)
(0.015, 0.96357481756888)
(0.02, 0.939642452605222)
(0.025, 0.904984588287098)
(0.03, 0.88647555882176)
(0.035, 0.857935412517365)
(0.04, 0.828161676414765)
(0.045, 0.81423302342588)
(0.05, 0.799611037022925)
(0.055, 0.792967900266247)
(0.06, 0.789989252128507)
(0.065, 0.785419281751758)
(0.07, 0.783213387255995)
(0.075, 0.78171575147004)
(0.08, 0.778121854334672)
(0.085, 0.778195990791145)
(0.09, 0.773367284376025)
(0.095, 0.776276435795401)
(0.1, 0.776118061749224)
(0.105, 0.773509431320769)
(0.11, 0.7721674447394)
(0.115, 0.770141793371259)
(0.12, 0.769890510378541)
(0.125, 0.768181932504691)
(0.13, 0.768463197970816)
(0.135, 0.767980791089438)
(0.14, 0.768624743272845)
(0.145, 0.769129960234898)
(0.15, 0.767185889872907)
(0.155, 0.76451614086641)
(0.16, 0.763597135128153)
(0.165, 0.764985143367184)
(0.17, 0.762010576434432)
(0.175, 0.762082976809109)
(0.18, 0.762681005792532)
(0.185, 0.761954213007711)
(0.19, 0.760230257975791)
(0.195, 0.760395576237545)
(0.2, 0.760400562426698)
(0.205, 0.760869010342264)
(0.21, 0.758107728047886)
(0.215, 0.757651311745867)
(0.22, 0.7583281424097)
(0.225, 0.755708904117756)
(0.23, 0.758038106462385)
(0.235, 0.756028633675693)
(0.24, 0.753130476002791)
(0.245, 0.754835266116217)
(0.25, 0.753682308451217)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 0.993211154408183)
(0.01, 0.982528706261878)
(0.015, 0.96119419549957)
(0.02, 0.938084982711339)
(0.025, 0.904127403493322)
(0.03, 0.883491514696613)
(0.035, 0.855150229063918)
(0.04, 0.823908664833249)
(0.045, 0.808560261557631)
(0.05, 0.789866323744205)
(0.055, 0.781169095772223)
(0.06, 0.776383659095848)
(0.065, 0.767938416347164)
(0.07, 0.758331210393911)
(0.075, 0.756627865440458)
(0.08, 0.746446933610162)
(0.085, 0.74135934748968)
(0.09, 0.732614151073426)
(0.095, 0.726945399703914)
(0.1, 0.719583126461675)
(0.105, 0.720829066554968)
(0.11, 0.711594373466194)
(0.115, 0.699938696388108)
(0.12, 0.697476706497176)
(0.125, 0.690590998948687)
(0.13, 0.689686886628668)
(0.135, 0.680815773786003)
(0.14, 0.681948382093995)
(0.145, 0.675524613325757)
(0.15, 0.668206477097926)
(0.155, 0.659334078056529)
(0.16, 0.657218665691577)
(0.165, 0.655729041035745)
(0.17, 0.652499555668288)
(0.175, 0.645800710081697)
(0.18, 0.641609828785437)
(0.185, 0.638429842277073)
(0.19, 0.636466595988368)
(0.195, 0.627482723826847)
(0.2, 0.630101989817678)
(0.205, 0.625460362889049)
(0.21, 0.619661433566945)
(0.215, 0.619338142529033)
(0.22, 0.613528092002575)
(0.225, 0.613022668683639)
(0.23, 0.609330976232567)
(0.235, 0.606944444444444)
(0.24, 0.599646035744911)
(0.245, 0.599782986674527)
(0.25, 0.595499795280421)
};


==> graphs/lambda.k10.B50.L15.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 11.74)
(0.050000, 21.97)
(0.075000, 15.49)
(0.100000, 12.67)
(0.125000, 11.36)
(0.150000, 10.40)
(0.175000, 9.75)
(0.200000, 9.24)
(0.225000, 8.77)
(0.250000, 8.34)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 10.09)
(0.050000, 20.91)
(0.075000, 18.02)
(0.100000, 15.76)
(0.125000, 14.39)
(0.150000, 13.32)
(0.175000, 12.53)
(0.200000, 11.89)
(0.225000, 11.42)
(0.250000, 11.05)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 13.46)
(0.050000, 23.09)
(0.075000, 17.94)
(0.100000, 16.01)
(0.125000, 15.37)
(0.150000, 15.02)
(0.175000, 14.87)
(0.200000, 14.75)
(0.225000, 14.66)
(0.250000, 14.51)
};


==> graphs/lambda.k10.B50.L15.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 1)
(0.05, 1)
(0.075, 1)
(0.1, 1)
(0.125, 1)
(0.15, 1)
(0.175, 1)
(0.2, 1)
(0.225, 1)
(0.25, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.998957448459739)
(0.05, 0.983456627547613)
(0.075, 0.985716646435205)
(0.1, 0.987607149019583)
(0.125, 0.988586755568859)
(0.15, 0.988625176138055)
(0.175, 0.988603199028305)
(0.2, 0.988587970433483)
(0.225, 0.988472712208328)
(0.25, 0.988295053493377)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.996374730502425)
(0.05, 0.900280632090428)
(0.075, 0.865543959699983)
(0.1, 0.861693727034622)
(0.125, 0.858505605173905)
(0.15, 0.85608679694812)
(0.175, 0.854366578470795)
(0.2, 0.852109251926716)
(0.225, 0.850507495138253)
(0.25, 0.849515384827879)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.996672121641809)
(0.05, 0.941624541437105)
(0.075, 0.890792472665552)
(0.1, 0.840009194490462)
(0.125, 0.794889742537256)
(0.15, 0.753004067991985)
(0.175, 0.716934449046329)
(0.2, 0.687767446029341)
(0.225, 0.660742151939817)
(0.25, 0.637600039843538)
};


==> graphs/lambda.k10.B50.L25.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 7.64)
(0.050000, 7.53)
(0.075000, 6.24)
(0.100000, 5.34)
(0.125000, 4.79)
(0.150000, 4.33)
(0.175000, 4.03)
(0.200000, 3.78)
(0.225000, 3.57)
(0.250000, 3.36)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 7.10)
(0.050000, 7.94)
(0.075000, 7.23)
(0.100000, 6.41)
(0.125000, 5.86)
(0.150000, 5.36)
(0.175000, 5.02)
(0.200000, 4.74)
(0.225000, 4.51)
(0.250000, 4.29)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025000, 8.29)
(0.050000, 8.40)
(0.075000, 7.30)
(0.100000, 6.63)
(0.125000, 6.36)
(0.150000, 6.20)
(0.175000, 6.15)
(0.200000, 6.13)
(0.225000, 6.13)
(0.250000, 6.12)
};


==> graphs/lambda.k10.B50.L25.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 1)
(0.05, 1)
(0.075, 1)
(0.1, 1)
(0.125, 1)
(0.15, 1)
(0.175, 1)
(0.2, 1)
(0.225, 1)
(0.25, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.936075273679081)
(0.05, 0.862801547717812)
(0.075, 0.862448485097417)
(0.1, 0.868648407244935)
(0.125, 0.874317828453959)
(0.15, 0.877161571495929)
(0.175, 0.879315846276571)
(0.2, 0.8798159280543)
(0.225, 0.881457119823486)
(0.25, 0.882016196770636)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.915526986088713)
(0.05, 0.804128587009796)
(0.075, 0.782629327509893)
(0.1, 0.778841956164648)
(0.125, 0.777645328797118)
(0.15, 0.776365834077466)
(0.175, 0.775530051627449)
(0.2, 0.773760301330785)
(0.225, 0.773004694782068)
(0.25, 0.772398588635966)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.915288348982904)
(0.05, 0.800104509613374)
(0.075, 0.755675398859013)
(0.1, 0.720804486025918)
(0.125, 0.690788445304576)
(0.15, 0.661178514716729)
(0.175, 0.636120953658245)
(0.2, 0.614195543503275)
(0.225, 0.594499679424425)
(0.25, 0.575584728089357)
};


==> graphs/lambda.k10.B50.L5.tot.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.999962139317845)
(0.05, 0.928256924072789)
(0.075, 0.77160811546325)
(0.1, 0.663881205024698)
(0.125, 0.589219379189329)
(0.15, 0.536199001677857)
(0.175, 0.489245036568184)
(0.2, 0.455901301350724)
(0.225, 0.425738590628478)
(0.25, 0.40167810381516)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.999957128345207)
(0.05, 0.928031311660429)
(0.075, 0.771426965904788)
(0.1, 0.663805862110083)
(0.125, 0.589109962523818)
(0.15, 0.53610746693173)
(0.175, 0.489161297915137)
(0.2, 0.455812508097566)
(0.225, 0.425650859549546)
(0.25, 0.40159554385153)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.99985328985665)
(0.05, 0.864719733677081)
(0.075, 0.694568073370007)
(0.1, 0.596146463843262)
(0.125, 0.527534495065475)
(0.15, 0.479824952297034)
(0.175, 0.436996582601463)
(0.2, 0.407369728890272)
(0.225, 0.37927217485959)
(0.25, 0.356688755625935)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=1,smooth,line width=1pt] coordinates {
(0.025, 0.999891150538805)
(0.05, 0.898439179907237)
(0.075, 0.695470124232552)
(0.1, 0.561897717575798)
(0.125, 0.459914550317272)
(0.15, 0.395518367248148)
(0.175, 0.345585074144274)
(0.2, 0.309993220529208)
(0.225, 0.276536992595816)
(0.25, 0.249038163985813)
};


==> graphs/lambda.k10.B50.L7.2.tex <==
% FOPTUW
\addplot [smooth,color=black,mark=x,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 1)
(0.01, 1)
(0.015, 1)
(0.02, 1)
(0.025, 1)
(0.03, 1)
(0.035, 1)
(0.04, 1)
(0.045, 1)
(0.05, 1)
(0.055, 1)
(0.06, 1)
(0.065, 1)
(0.07, 1)
(0.075, 1)
(0.08, 1)
(0.085, 1)
(0.09, 1)
(0.095, 1)
(0.1, 1)
(0.105, 1)
(0.11, 1)
(0.115, 1)
(0.12, 1)
(0.125, 1)
(0.13, 1)
(0.135, 1)
(0.14, 1)
(0.145, 1)
(0.15, 1)
(0.155, 1)
(0.16, 1)
(0.165, 1)
(0.17, 1)
(0.175, 1)
(0.18, 1)
(0.185, 1)
(0.19, 1)
(0.195, 1)
(0.2, 1)
(0.205, 1)
(0.21, 1)
(0.215, 1)
(0.22, 1)
(0.225, 1)
(0.23, 1)
(0.235, 1)
(0.24, 1)
(0.245, 1)
(0.25, 1)
};
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 1.00002794310783)
(0.01, 1.00001236690123)
(0.015, 1)
(0.02, 0.999227193817551)
(0.025, 0.999313756619176)
(0.03, 0.998310109694634)
(0.035, 0.995202556712633)
(0.04, 0.991702338660072)
(0.045, 0.990277632268203)
(0.05, 0.990132674623413)
(0.055, 0.988975041488395)
(0.06, 0.989502852019306)
(0.065, 0.988174945070154)
(0.07, 0.98757278671637)
(0.075, 0.986635972617677)
(0.08, 0.986817747376494)
(0.085, 0.986818525508594)
(0.09, 0.986699506446433)
(0.095, 0.985797316945434)
(0.1, 0.9862292550303)
(0.105, 0.985770153809786)
(0.11, 0.985562463081035)
(0.115, 0.98556704455795)
(0.12, 0.985236553772872)
(0.125, 0.985237553624775)
(0.13, 0.98479669428798)
(0.135, 0.984563665028285)
(0.14, 0.984511275478244)
(0.145, 0.985243808113719)
(0.15, 0.983964554307424)
(0.155, 0.984110752544887)
(0.16, 0.983352065286912)
(0.165, 0.984280850690042)
(0.17, 0.98318493666704)
(0.175, 0.983102997986833)
(0.18, 0.982985271488239)
(0.185, 0.982839280084254)
(0.19, 0.982284177655324)
(0.195, 0.981596671379773)
(0.2, 0.983029220869002)
(0.205, 0.981815164364669)
(0.21, 0.981225074941396)
(0.215, 0.981452187932587)
(0.22, 0.982104810943074)
(0.225, 0.980784236258581)
(0.23, 0.980622065136308)
(0.235, 0.979898840045323)
(0.24, 0.97997876118061)
(0.245, 0.980004868462456)
(0.25, 0.979630945510438)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 1.00002794310783)
(0.01, 1.00001236690123)
(0.015, 0.999760608586172)
(0.02, 0.997216777734222)
(0.025, 0.997265268915223)
(0.03, 0.992423023167168)
(0.035, 0.974678156483222)
(0.04, 0.954761426544984)
(0.045, 0.940618124672603)
(0.05, 0.913280519293646)
(0.055, 0.902087388787179)
(0.06, 0.891093878173945)
(0.065, 0.870356914240238)
(0.07, 0.873918566178075)
(0.075, 0.862137275095414)
(0.08, 0.857632839615278)
(0.085, 0.859877869927702)
(0.09, 0.855734617835675)
(0.095, 0.853287163015891)
(0.1, 0.851657342442869)
(0.105, 0.847277965921685)
(0.11, 0.847002730099302)
(0.115, 0.845727336904614)
(0.12, 0.844371546462567)
(0.125, 0.843515551381462)
(0.13, 0.842346853350098)
(0.135, 0.843553123744165)
(0.14, 0.841619283958946)
(0.145, 0.843920892216625)
(0.15, 0.841225737191396)
(0.155, 0.83922167310734)
(0.16, 0.839527698362841)
(0.165, 0.839443659706982)
(0.17, 0.837586173052492)
(0.175, 0.837434027966701)
(0.18, 0.838349087711585)
(0.185, 0.837828446465825)
(0.19, 0.838856086707052)
(0.195, 0.835637615290326)
(0.2, 0.838160024123578)
(0.205, 0.837741349498775)
(0.21, 0.835708957633891)
(0.215, 0.835555820112186)
(0.22, 0.835698231151899)
(0.225, 0.836079559484419)
(0.23, 0.834880774330873)
(0.235, 0.834306763841678)
(0.24, 0.834610176674892)
(0.245, 0.833709946506284)
(0.25, 0.833080280999301)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005, 1.00002794310783)
(0.01, 1.00001236690123)
(0.015, 0.999911336513397)
(0.02, 0.998202385619085)
(0.025, 0.998217815697561)
(0.03, 0.99565880310025)
(0.035, 0.985928702057129)
(0.04, 0.973719888025508)
(0.045, 0.966453640649555)
(0.05, 0.951073734474884)
(0.055, 0.943613557324496)
(0.06, 0.934789866269864)
(0.065, 0.913766630335115)
(0.07, 0.915202929801741)
(0.075, 0.895535227479251)
(0.08, 0.88643641198238)
(0.085, 0.891321302905997)
(0.09, 0.880829491500123)
(0.095, 0.868202177647072)
(0.1, 0.863445374361121)
(0.105, 0.847877514033708)
(0.11, 0.841943668217616)
(0.115, 0.83748017108924)
(0.12, 0.82282420120271)
(0.125, 0.814561712343098)
(0.13, 0.817301282922067)
(0.135, 0.80916257071316)
(0.14, 0.797336529658363)
(0.145, 0.798930112009553)
(0.15, 0.790207202219321)
(0.155, 0.780334412894479)
(0.16, 0.773871844947857)
(0.165, 0.772634087389686)
(0.17, 0.759378987253231)
(0.175, 0.752796670112629)
(0.18, 0.758240822158716)
(0.185, 0.747322452758045)
(0.19, 0.740572934982932)
(0.195, 0.733199432336437)
(0.2, 0.737758798456196)
(0.205, 0.729880251538667)
(0.21, 0.719794533299055)
(0.215, 0.720301020414625)
(0.22, 0.712172738196784)
(0.225, 0.709710356066966)
(0.23, 0.706407327435238)
(0.235, 0.695760356052313)
(0.24, 0.694644680777192)
(0.245, 0.687956492569658)
(0.25, 0.682051936406407)
};


==> graphs/lambda.k10.B50.L7.lat.tex <==
% POValue
\addplot [smooth,color=blue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005000, 5.15)
(0.010000, 6.02)
(0.015000, 7.36)
(0.020000, 11.01)
(0.025000, 11.63)
(0.030000, 17.87)
(0.035000, 25.24)
(0.040000, 31.46)
(0.045000, 30.34)
(0.050000, 27.33)
(0.055000, 26.61)
(0.060000, 24.25)
(0.065000, 21.22)
(0.070000, 21.40)
(0.075000, 19.11)
(0.080000, 18.10)
(0.085000, 18.66)
(0.090000, 17.86)
(0.095000, 16.73)
(0.100000, 16.30)
(0.105000, 15.21)
(0.110000, 14.94)
(0.115000, 14.59)
(0.120000, 14.01)
(0.125000, 13.62)
(0.130000, 13.71)
(0.135000, 13.37)
(0.140000, 12.96)
(0.145000, 12.99)
(0.150000, 12.70)
(0.155000, 12.39)
(0.160000, 12.25)
(0.165000, 12.25)
(0.170000, 12.01)
(0.175000, 11.82)
(0.180000, 11.99)
(0.185000, 11.69)
(0.190000, 11.69)
(0.195000, 11.43)
(0.200000, 11.63)
(0.205000, 11.41)
(0.210000, 11.23)
(0.215000, 11.22)
(0.220000, 11.15)
(0.225000, 10.99)
(0.230000, 10.98)
(0.235000, 10.76)
(0.240000, 10.76)
(0.245000, 10.80)
(0.250000, 10.63)
};
% POWork
\addplot [smooth,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005000, 5.06)
(0.010000, 5.83)
(0.015000, 6.91)
(0.020000, 9.81)
(0.025000, 10.36)
(0.030000, 14.40)
(0.035000, 19.46)
(0.040000, 23.84)
(0.045000, 24.13)
(0.050000, 24.36)
(0.055000, 25.11)
(0.060000, 24.03)
(0.065000, 22.54)
(0.070000, 22.40)
(0.075000, 21.13)
(0.080000, 20.61)
(0.085000, 20.95)
(0.090000, 20.37)
(0.095000, 19.18)
(0.100000, 19.28)
(0.105000, 18.50)
(0.110000, 18.02)
(0.115000, 17.80)
(0.120000, 17.11)
(0.125000, 16.67)
(0.130000, 16.88)
(0.135000, 16.36)
(0.140000, 16.03)
(0.145000, 16.14)
(0.150000, 15.59)
(0.155000, 15.68)
(0.160000, 15.28)
(0.165000, 15.12)
(0.170000, 14.73)
(0.175000, 14.57)
(0.180000, 14.72)
(0.185000, 14.28)
(0.190000, 14.02)
(0.195000, 14.00)
(0.200000, 14.12)
(0.205000, 13.72)
(0.210000, 13.44)
(0.215000, 13.50)
(0.220000, 13.34)
(0.225000, 13.08)
(0.230000, 13.13)
(0.235000, 12.63)
(0.240000, 12.73)
(0.245000, 12.71)
(0.250000, 12.45)
};
% POLen
\addplot [smooth,color=red,mark=star,mark size=2pt,mark repeat=5,smooth,line width=1pt] coordinates {
(0.005000, 5.34)
(0.010000, 6.50)
(0.015000, 8.29)
(0.020000, 13.05)
(0.025000, 13.81)
(0.030000, 20.76)
(0.035000, 28.48)
(0.040000, 34.32)
(0.045000, 33.49)
(0.050000, 31.33)
(0.055000, 31.16)
(0.060000, 29.01)
(0.065000, 26.33)
(0.070000, 26.34)
(0.075000, 24.38)
(0.080000, 23.65)
(0.085000, 24.07)
(0.090000, 23.38)
(0.095000, 22.27)
(0.100000, 21.79)
(0.105000, 20.61)
(0.110000, 20.46)
(0.115000, 20.28)
(0.120000, 19.62)
(0.125000, 19.34)
(0.130000, 19.32)
(0.135000, 18.93)
(0.140000, 18.70)
(0.145000, 18.66)
(0.150000, 18.48)
(0.155000, 18.27)
(0.160000, 18.16)
(0.165000, 18.08)
(0.170000, 17.90)
(0.175000, 17.76)
(0.180000, 17.79)
(0.185000, 17.69)
(0.190000, 17.66)
(0.195000, 17.52)
(0.200000, 17.61)
(0.205000, 17.44)
(0.210000, 17.37)
(0.215000, 17.40)
(0.220000, 17.40)
(0.225000, 17.23)
(0.230000, 17.32)
(0.235000, 17.18)
(0.240000, 17.26)
(0.245000, 17.25)
(0.250000, 17.26)
};

